Publication Bias in Asset Pricing Research

Researchers are more likely to share notable findings. As a result, published findings tend to overstate the magnitude of real-world phenomena. This bias is a natural concern for asset pricing research, which has found hundreds of return predictors and little consensus on their origins. Empirical evidence on publication bias comes from large scale meta-studies. Meta-studies of cross-sectional return predictability have settled on four stylized facts that demonstrate publication bias is not a dominant factor: (1) almost all findings can be replicated, (2) predictability persists out-of-sample, (3) empirical $t$-statistics are much larger than 2.0, and (4) predictors are weakly correlated. Each of these facts has been demonstrated in at least three meta-studies. Empirical Bayes statistics turn these facts into publication bias corrections. Estimates from three meta-studies find that the average correction (shrinkage) accounts for only 10 to 15 percent of in-sample mean returns and that the risk of inference going in the wrong direction (the false discovery rate) is less than 10%. Meta-studies also find that $t$-statistic hurdles exceed 3.0 in multiple testing algorithms and that returns are 30 to 50 percent weaker in alternative portfolio tests. These facts are easily misinterpreted as evidence of publication bias effects. We clarify these misinterpretations and others, including the conflating of ``mostly false findings'' with ``many insignificant findings,'' ``data snooping'' with ``liquidity effects,'' and ``failed replications'' with ``insignificant ad-hoc trading strategies.'' Meta-studies outside of the cross-sectional literature are rare. The four facts from cross-sectional meta-studies provide a framework for future research. We illustrate with a preliminary re-examination of equity premium predictability.

==> backup.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Publication Bias in Other Fields}\label{sec:conclusion}

In a 2005 opinion piece in PLoS Medicine, \citeauthor{ioannidis2005most} proclaimed ``[i]t can be proven that most claimed research findings are false.''  
He provides  six ``corollaries'' detailing the causes of widespread scientific failure, and even has a section titled ``Most Research Findings Are False for Most Research Designs in Most Fields.''  With such bold language, certainly the argument must be foolproof?


More than 10 years later, \citet{leek2017most} and \citet{fanelli2018science} review the empirical evidence.  Their reviews parallel Facts 1-3 from Section \ref{sec:facts}: 
\begin{enumerate}
    \item Without common data sources like CRSP and Compustat, replication as in \citet{ChenZimmermann2021} is not so easy in biomedical research. Nevertheless, anonymous surveys, random lab audits, and image analyses find intentional author errors in biomedical research are rare. 
    
    \item Out-of-sample replication studies are hard to find for biomedical research.  But results from psychology show that replication depends on the field of research. Social psychology effects drop by more than 50\% out-of-sample, but effects from  cognitive psychology are still mostly there.
    
    \item p-values are extremely small, much smaller than 0.05.  Using methods like those in Section \ref{sec:gap}, \citet{jager2014estimate} find a false discovery rate of just 14\% in top medical journals. \citet{fanelli2018science} acknowledge potential problems with this analysis, but also finds ``there is no alternative analysis that suggests that P-hacking is severely distorting the scientific literature.''
    
\end{enumerate}
Fact 4 is less relevant for biomedical research, as there does not seem to be a belief in a strong factor structure.  Overall, these facts suggest that publication bias is a minor issue in the biomedical research, though more work could be done, especially in out-of-sample replications.

As in Section \ref{sec:mis}, loose language is important.  Ioannidis's ``corollaries'' come with no proofs, so they would be more precisely described as ``hypotheses.''  Ioannidis's ``proof'' depends on parameter values that are not universally accepted (e.g., \citet{christensen2018transparency}). Thus, ``it can be proven that most claimed research findings are false'' would in more precise language be ``under certain parameter values, most claimed research findings are false.''  



In  any  re-analysis of asset pricing research, researchers should be careful to use precise language and to avoid over-extending.  Precise language is important, especially in academic publications.  In everyday life, loose language causes confusion.  In academic publications, loose language is written down to cause confusion for future generations.  16 years after its  publication,  \citet{ioannidis2005most} still receives  1,000 Google scholar citations per year.    How will future generations understand publication bias in biomedical research?  How will they understand publication bias  in asset pricing?


% Google Scholar counted 1,167 citations to \citet{ioannidis2005most} in 2021 alone.  


%\citet{harvey2016and} and \citet{Hou2020Replicating} have 234 and 235 citations in 2021, respectively.


% Google Scholar counted 1,167 citations to \citet{ioannidis2005most} in 2021 alone,  far outshadowing the 20 citations to  \citet{jager2014estimate} or the 206 to \citet{fanelli2009many}.  One wonders how future generations will read these papers, and how many will get lost in the language.

% \citet{harvey2016and} and \citet{Hou2020Replicating} seems to be following in \citet{ioannidis2005most}'s footsteps, with 234 and 235 citations in 2021, respectively, compared to 23 for \citet{chen2020publication}.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}\label{sec:conclusion}


Publication bias may seem like a slippery topic, but its essence is seen in a simple decomposition:
\begin{align}
    \text{Reported effect} = \text{True effect} + \text{Author error} + \text{Sampling error}.
\end{align}
Publication bias selects for large reported effects, which selects for large author errors and sampling errors.  As a result, published reported effects are upward biased compared to the corresponding true effects.

Meta-studies can measure author errors and sampling errors. Four facts from cross-sectional predictability illustrate how.  These facts show that publication bias is a rather small problem in the cross-section, and provide a framework for understanding publication bias in other literatures.  

Meta-studies need to be read with caution.  They cover a lot of ground, making rigorous language difficult. A paper may say ``most findings are likely false'' when the rigorous language is ``many predictors are insignificant.''   ``Replications fail due to microcaps'' may very well mean ``predictors that were insignificant replicate correctly.''
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Illustration: Equity Premium Predictability}\label{sec:ts}

Outside of cross-sectional predictability, empirical evidence on publication bias is scarce.  The four facts in Section \ref{sec:facts} provide a framework for future research.  We end our review by illustrating how to apply these facts to equity premium predictability.  This analysis is very preliminary---it is only meant as an illustration.

Equity premium predictability refers to predicting the aggregate stock market return in excess of a risk-free rate (\citet{Rapach2022AssetPricing}).  There are multiple ways to measure this type of predictability.  We focus on ``real-time forecasting performance,'' that is, whether using a predictor would lead to smaller forecast errors when compared to the historical mean in real-time.  Real-time performance is analogous to the long-short returns studied in Sections \ref{sec:facts} and \ref{sec:gap}.   The equity premium literature refers to real-time performance as ``out-of-sample,'' but we reserve this term for ``after the original paper's sample periods.''

\citet{Goyal2008A} study real-time performance of 17 predictors.  In on-going work,  \citet{Goyal2021A} add another 29 predictors.  These studies suggest four preliminary facts:
\begin{enumerate}
    \item \textbf{Real-time equity premium prediction seems to replicate poorly.}  \citet{Goyal2021A} find that, of 21 predictors that showed real-time out-performance, only 10 showed real-time out-performance in \citet{Goyal2021A}'s replications. Some of the differences in performance was due to changes in the start date of out-of-sample evaluation.  This fragility suggests that either author errors or sampling errors in Equation \eqref{eq:intro} are large, though a closer investigation would be necessary to pin down which is the main driver.
    
    \item \textbf{Little evidence supports equity premium predictability persisting out-of-sample.}  
\end{enumerate}






We illustrate how to use the four facts using data and results from \citet{Goyal2008A} and \citet{Goyal2021A}.   
These papers re-examine predictors of the equity premium---that is, predictors of the aggregate stock market return in excess of a risk-free rate.  \citet{Goyal2008A} re-examine 17 predictors.    The analysis that follows is very preliminary---it is only meant as an illustration.

The equi




\textbf{Fact \#2: Little evidence supports equity premium predictability persisting out-of-sample.} As emphasized in Sections \ref{sec:facts-oos} and \ref{sec:mis-oos}, the cleanest out-of-sample tests zoom  in on time periods near the end of the original samples (\citet{Mclean2016Does}).  Unfortunately, such a test is likely impossible, as the equity premium data is an order of magnitude  smaller than the cross-sectional data.   The equity premium is often predicted at the one year horizon or even longer, compared the the ubiquitous monthly horizon in cross-sectional predictability.

Nevertheless, indirect evidence suggests that out-of-sample predictability is poor.  \citet{Goyal2008A} find that  most predictors are insignificant in samples that combine the original in-sample periods with out-of-sample data.  Goyal and Welch also find that predictors under-perform the naive historical mean forecast in expanding window tests, especially in recent data.  Their recent update (\citet{Goyal2021A}) finds similar results in the updated  sample.   

These results suggest that either predictability declines out-of-sample or  the sampling error term in Equation \eqref{eq:intro} is large.  But due to the long forecasting horizons in equity premium predictability, it is  difficult to separate the two effects using out-of-sample tests.

An important caveat is that predictability in the equity premium literature means something different than 


\textbf{Fact \#3: Equity premium prediction t-stats are somewhat larger than 2.0.}  The mean t-stat is 2.8 in \citet{Goyal2021A}'s replications, and the 90th percentile is 4.0.  These t-stats are  much closer to 2.0 than the t-stats from the cross-section, as seen in Figure \ref{fig:ts_hist}.  But they are still far enough from 2.0 to imply that sampling error has a minority role.

\begin{figure}[h!]
    \caption{
    Distribution of  t-statistics in Equity Premium Predictability.  Equity premium t-stats (red)  use \citet{Goyal2021A}'s replications (their Table 2).  Cross-sectional t-stats (grey) are replicated by \citet{ChenZimmermann2021}.  Equity premium t-stats somewhat larger 2.0, implying a much larger role for publication bias compared to the cross-section.
    }
    \label{fig:ts_hist}
    \vspace{.10in}
    \centering     
                                \includegraphics[width=5in]{exhibits/ts-filling-the-gap.pdf}
                                                               
\end{figure}

A t-stat of 2.8 is significant at the 0.5\% level.  This means it would take 1/0.005 $=$ 200 draws to generate the average t-stat in the equity premium literature, far fewer than the 16,000 draws it would take to generate the average t-stat in the cross-section.  

Nevertheless, 200 draws 



These small t-stats also imply shrinkage and FDR estimates are larger than  


If there was no predictability, it would take just 370 draws to generate the average t-stat of 3.0.  

These numbers are much lower than in the cross-sectional asset pricing literature. Such a distribution is consistent with publication bias in time-series predictability because values could still realistically be the result of profession-wide p-hacking.  These results are also more consistent with larger shrinkage and FDR estimates.



\textbf{Fact \#4: Predictors are weakly dependent.} This has not been documented comprehensively in the literature but we used the \cite{Goyal2008A} data\footnote{We used the updated data with values updated throughout 2021, available on Goyal's website.} to calculate pairwise predictor correlation coefficients between up to 17 predictors studied in that paper.
Figure \ref{fig:ts_cors} shows that these correlations are centered around zero, similar to cross-sectional predictors (Figure \ref{fig:cor}).   This implies that the predictors are distinct, and that standard multiple testing estimates can be applied.

\begin{figure}[h!]
    \caption{
                                                {Pairwise predictor correlations} 
                                }
    \label{fig:ts_cors}
    \vspace{.10in}
    \centering     
                                \includegraphics[width=5in]{exhibits/fig_ts_correlations.pdf}
                                                               
\end{figure}

This finding is surprising given that all of these predictors aim to forecast the same equity premium.  However, it is consistent with both the fact that journals are much more likely to publish novel results,  and the fact that combination forecasts seem to work rather well (\citet{Rapach2013Forecasting}).  Combination forecasts rely on diversification effects, which would not occur if predictors are highly correlated.


Overall, the literature on time-series predictability is more  consistent with large publication bias effects than the cross-sectional asset pricing literature.  There is little-to-no evidence supporting out-of-sample predictability (in the sense of \citet{Mclean2016Does}).  t-statistics are much closer to 2, much larger shrinkage corrections and FDRs.  Clearly establishing publication bias corrections remains an area for future research.  The four facts we establish for the cross-section (Section \ref{sec:facts}) provide an outline for this future work.



